Visually Informed Binaural Audio Generation without Binaural Audios

Stereophonic audio, especially binaural audio, plays an essential role in immersive viewing environments. Recent research has explored generating visually guided stereophonic audios supervised by multi-channel audio collections. However, due to the requirement of professional recording devices, existing datasets are limited in scale and variety, which impedes the generalization of supervised methods in real-world scenarios. In this work, we propose PseudoBinaural, an effective pipeline that is free of binaural recordings. The key insight is to carefully build pseudo visual-stereo pairs with mono data for training. Specifically, we leverage spherical harmonic decomposition and head-related impulse response (HRIR) to identify the relationship between spatial locations and received binaural audios. Then in the visual modality, corresponding visual cues of the mono data are manually placed at sound source positions to form the pairs. Compared to fully-supervised paradigms, our binaural-recording-free pipeline shows great stability in cross-dataset evaluation and achieves comparable performance under subjective preference. Moreover, combined with binaural recordings, our method is able to further boost the performance of binaural audio generation under supervised settings.

==> sections/experiments.tex <==
% Table 1%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\setlength{\tabcolsep}{6.5pt}
\begin{table*}[t] %\footnotesize
\begin{center}
\caption{Quantitative results of binaural audio generation on FAIR-Play and MUSIC-Stereo dataset with five different evaluation metrics.  Except for SNR, the lower the score, the better the results. The upper half shows the results of standard benchmarks and our PseudoBinaural method. 
%
%Since without the supervision of ground-truth binaural audio, it's reasonable that ours is slightly worse than Mono2Binaural~\cite{gao20192}. 
%
The lower half shows the augmentation results and our ablation studies on different binaural decoding schemes~\ref{sec:3.1.2}. Once including binaural audio to train, our method can outperform the supervised method~\cite{gao20192} by a large margin or previous augmentation method Sep-Stereo~\cite{zhou2020sep}. 
Moreover, PseudoBinaural constructing binaurals from ambisonics with HRIR  achieves the best performance among three decoding methods. }
\label{table:exp1}
\begin{tabular}{lcccccccccc}
\toprule
 & \multicolumn{5}{c}{FAIR-Play }& \multicolumn{5}{c}{MUSIC-Stereo} \\
\cmidrule(lr){2-6} \cmidrule(lr){7-11}
Method & $\text{STFT} $ & $\text{ENV} $ & $\text{Mag} $ & $\mathcal{D}_{phase} $ & $\text{SNR} \uparrow $ & $\text{STFT} $ & $\text{ENV}$ & $\text{Mag} $ & $\mathcal{D}_{phase} $  & $\text{SNR} \uparrow$ \\

\midrule
Mono-Mono &1.024 &0.145 &2.049 &1.571 &4.968 &1.014 &0.144 &2.027 &1.568 &7.858 \\
Mono2Binaural~\cite{gao20192}  &0.917 &0.137 &1.835 &1.504 &5.203 &0.942 &0.138 &1.885 &1.550 &8.255 \\

\textbf{PseudoBinaural} (w/o sep.) &0.951 &0.140 &1.914 &1.539 & 5.037 &0.953 &0.139 &1.902 &1.564 &8.129 \\
\textbf{PseudoBinaural} (Ours) & 0.944 & 0.139 & 1.901 & 1.522 & 5.124 &0.943 &0.139 &1.886 &1.562 &8.198 \\
\hline
\hline
Sep-Stereo~\cite{zhou2020sep} &0.906 &0.136 &1.811 &1.495 &5.221 &0.929 &0.135 &1.803 &1.544 &8.306 \\
Augment-HRIR  &0.896 &0.137 &1.791 &1.472 &5.255 &0.940 &0.138 &1.866 &1.550 &8.259 \\
Augment-ambisonic &0.912 &0.139 &1.823 &1.477 &5.220 &0.909 &0.137 &1.817 &1.546 &8.277 \\
\textbf{Augment-PseudoBinaural} &\textbf{0.878} &\textbf{0.134} &\textbf{1.768} &\textbf{1.467} &\textbf{5.316} &\textbf{0.891} &\textbf{0.132} &\textbf{1.762} &\textbf{1.539} &\textbf{8.419} \\

\bottomrule
\end{tabular}
\end{center}

\vspace{-10pt}
\end{table*}
%\setlength{\tabcolsep}{2pt}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{Experiments}


% \textbf{Implementation Details.} 
% The detailed network structure and pre-processing of the audios are directly borrowed from that of Mono2Binaural~\cite{gao20192}. The complex spectrums are of size $257\times 64\times 2$, and the visual input is a $224\times 448\times 3$ image. The experiments are carried out on PyTorch~\cite{NIPS2019_9015}.

\subsection{Datasets} 

We emphasize creating binaurals for music, which is an important scenario for stereo production. We will at first show our analysis on the FAIR-Play dataset, then introduce other datasets we use.

\noindent\textbf{Revisiting FAIR-Play.}
Collected in a music room, FAIR-Play~\cite{gao20192} is one of the most influential datasets in this field.% of visually informed binaural audio creation.
However, by carefully examining the dataset, we find that the original train-test splits are somewhat problematic. The whole dataset contains $1,871$  clips cut from several different long camera recordings with  approximately the same camera view and scene layouts. 
%Within each recorded video, the camera view and scene layouts are approximately the same.
The clips are randomly divided into 10 different train-test splits. As a result, the scenes within train and test splits are overlapped, probably originate from the same recording. 
%when the dataset was recorded. 
This would lead to serious overfitting problems. The models might learn layouts of the room instead of visual-stereo association that we desired.
%We have validated in the section below that 
%The traditional training pipelines might fail to learn the association between sound sources and stereo, but memorize the layout of the room instead. 

%Particularly, the model can still make reasonable prediction when the instruments are masked out.

%As training and testing on the original splits 
In order to evaluate the true generalization ability of different models on this dataset, we take efforts to re-organize the FAIR-Play dataset through reconstructing the original videos and re-splitting them.
%to avoid overlapped scenes in train and test set. 
%
Specifically, we first run a clustering algorithm on all the clips to roughly group them according to the scenes. Then by matching the first and last frame of each clip within groups, we find the original order of the clips and concatenate them to recover the recorded videos. Finally, we select the videos whose scenes are completely absent in other videos as the validate and test sets.
In this way, we create 5 different splits in which train and test sets are not overlapped.
%, we will release the information about the splits.
In our experiments, we re-train all supervised models (including Mono2Binaural~\cite{gao20192} and Sep-Stereo~\cite{zhou2020sep}) and report the average results on the five splits. Please be noted that our model is also trained on this dataset, using only the solo part and \emph{mono audios}.
%Please be noted that the model we propose in this paper does not require training on collected data, thus our model is directly tested on the test splits. 



\noindent\textbf{MUSIC-Stereo}~\cite{zhao2018sound,zhao2019sound}. %For building the pseudo visual-stereo pairs, the mono videos we leverage are selected from the MUSIC dataset~\cite{zhao2018sound} and its expansion MUSIC21~\cite{zhao2019sound}, which are originally collected for visually guided sound separation. 
Containing 21 different types of instruments, MUSIC(21) is originally collected for visually guided sound separation. We select all the videos with binaural audio from MUSIC(21) and MUSIC-duet~\cite{zhao2018sound}
to form a new dataset MUSIC-Stereo. Composed of solo and duet parts, it includes $1,120$ unique videos of different musical performances. MUSIC-Stereo lasts 49.7 hours in total, which is 10 times larger than the FAIR-Play dataset. 
Following the post-processing steps in \cite{gao20192}, we cut these videos into $17,940$ 10s clips and split them into training, validation, and test sets in an 8:1:1 ratio. Similar to FAIR-Play, only the solo part and \emph{mono audios} are exploited for our model's training. 
%Notably, we hold out 200 10s video clips containing binaurals from its duet part (in MUSIC \cite{zhao2018sound}) as an extra evaluation set.
%Our training samples are selected from this dataset for all of our evaluations. 
%The frontal mapping $f_{v2a}$ is defined in supplementary materials.

\noindent\textbf{YT-Music}~\cite{morgado2018self}. This dataset is collected from 360\degree videos on YouTube in the ambisonic format. %It contains a large variety of instruments and scenes, thus is the most challenging dataset. 
The audios are transferred to binaural in the same way as our decoding scheme. 
%Different from FAIR-Play and MUSIC-Stereo, 
With distinct vision configurations and stereo audio characteristics, YT-MUSIC is the most challenging dataset.%, making it a good evaluation dataset to demonstrate a method's generalization ability.
%When directly building the visual-stereo pair for this dataset, the azimuth range of mapping $f_{v2a}'$ is defined as 360\degree.

%These metrics focus on the absolute similarity between generated audios and ground truth, which may accidentally focus less on the sound localization accuracy in the audio domain. Moreover, such a metric is highly sensitive to the sliding window size during testing.



%\subsection{Implementation Details}
%Following \cite{gao20192}, we use Python package audiolab to resample the audio at 16kHz, which significantly accelerates the IO process during training. Besides, our detailed network structure and training procedures are all the same as Mono2Binaural~\cite{gao20192} and Sep-Stereo~\cite{zhou2020sep}. The complex spectrums are of size $257 \times 64 \times 2$, and the visual input is $224 \times 448 \times 3$ images. For testing, we find the hop length of sliding window will not affect the inference performance after fixing the audio normalization bug presented in~\cite{gao20192}. Hence, the sliding window is set as 0.1s for all the experiments.

% Table 2
\begin{table*}[t] %\footnotesize
\setlength{\tabcolsep}{8pt}
\begin{center}
\caption{Cross-dataset evaluation results on five metrics. While the model trained on FAIR-Play is used for testing on the others, the model trained on MUSIC-Stereo is for the evaluation on FAIR-Play. PseudoBinaural presents better generalization ability than the supervised method Mono2Binaural on all datasets.
%Our methods are all trained on mono data, but for evaluation on FAIR-Play, the self-created visual information is placed in a 360\degree manner while the others are frontal-view. Results show that we can outperform theirs on all datasets.
}
\label{table:exp2}
\begin{tabular}{lcccccccccc}
\toprule
 & \multicolumn{5}{c}{Mono2Binaural~\cite{gao20192}} & \multicolumn{5}{c}{\textbf{PseudoBinaural (Ours)}} \\
\cmidrule(lr){2-6} \cmidrule(lr){7-11}
Dataset & $\text{STFT} $ & $\text{ENV} $ & $\text{Mag} $ & $\mathcal{D}_{phase} $ & $\text{SNR} \uparrow $ & $\text{STFT} $ & $\text{ENV}$ & $\text{Mag} $ & $\mathcal{D}_{phase} $  & $\text{SNR} \uparrow$ \\

\midrule
FAIR-Play  &0.996 &0.142 &1.993 &1.562 &5.876 &\textbf{0.959} &\textbf{0.140} &\textbf{1.917} &\textbf{1.496} &\textbf{6.057} \\
MUSIC-Stereo  &0.971 &0.140 &1.942 &1.552 &7.933 &\textbf{0.952} &\textbf{0.139} &\textbf{1.904} &\textbf{0.574} & \textbf{8.099}\\
YT-MUSIC  &0.717 &0.118 &1.435 &1.597 &9.214  &\textbf{0.653} &\textbf{0.111} &\textbf{1.306} &\textbf{1.357} & \textbf{9.848} \\

\bottomrule
\end{tabular}
\end{center}
\vspace{-15pt}
\end{table*}

\subsection{Evaluation Metrics}
\noindent\textbf{Previous Metrics.} 
%
The evaluation protocol within this field is basically the STFT distance and the envelope distance (ENV) between recovered audios and recorded ones~\cite{morgado2018self,gao20192}. The STFT distance represents the mean square error computed on predicted spectrums, and the ENV distance is performed on raw audio waves through Hilbert transform~\cite{smith2007mathematics}. To evaluate the predicted binaural audios more comprehensively, we also adopt two widely-used metrics \emph{Magnitude Distance (Mag)} and \emph{Signal-to-noise Ratio (SNR)} from \cite{morgado2018self}. The Mag distance reflects the $L2$ deviation on the magnitude of spectrums and SNR is operated on the waveform directly. 
%Moreover, another new metric \emph{Difference Phase Distance} is further proposed.

\noindent\textbf{Newly Proposed Metric.} 
In 3D audio sensation, audiences care more about sensing the source direction, where the phase of binaural audio is the key.
As illustrated in \cite{neurals}, phase errors will introduce perceivable distortions but are always neglected during the optimization. Inspired by this, we further propose a new metric named \textit{Difference Phase Distance} ($\mathcal{D}_{phase}$), which is performed on the Time-Frequency domain. Note that, the binaural audio is completely determined by the difference between left and right spectrums~\ref{sec:3.3.2}. Hence, $\mathcal{D}_{phase}$ is to evaluate the phase distortion between the ground-truth difference $S_D$ and the predicted one $\Tilde{S_D} = \mathcal{M} * S_m$:
%Specifically, it takes the phase difference between the left spectrum $S_L = \text{STFT}(l(t))$ and right spectrum $S_R = \text{STFT}(r(t))$, and compute the difference between that of the gt and the predicted spectrum $\Tilde{S_L}$ and $\Tilde{S_R}$:
\begin{align}
\label{eq:10}
    \mathcal{D}_{phase} = \| \text{phase}(S_D) - \text{phase}(\Tilde{S_D}) \|_2,
\end{align}
where the phase is represented by the angle values, thus $\mathcal{D}_{phase} \in [0, 2\pi]$. It's worth emphasizing that $\mathcal{D}_{phase}$ is sensitive to the audio directions, \ie, switching left and right channels would bring a significant change on this metric.
%Note that, the phase is sensitive to the sound location. If we just swap the left and right channel of ground-truth stereo audio as the predicted ones, the phase distance value $\mathcal{D}_{phase}$ will be very large, indicating the bad performance of such trivial solution.


\subsection{Quantitative Results}
\noindent\textbf{Binaural-Recording-Free Evaluation.} 
%
Since no binaural-recording-free method has been proposed before, supervised method \emph{Mono2Binaural}~\cite{gao20192} whose backbone we borrow from, can be served as our baseline and upper bound. The evaluation is made on our newly-split FAIR-Play~\cite{gao20192} and MUSIC-Stereo.
%In this setting, their model is trained and tested on the original train-test split of FAIR-Play and YT-MUSIC, while ours are trained on MUSIC21 monos only.
For comparison, \emph{Mono2Binaural} is trained with both visual frames and binaural audio, whereas our method \emph{PseudoBinaural} only leverages frames and mono audio to do the training. Please be noted that we do not rely on an extra dataset.
%
The result of \emph{Mono-Mono} is also listed, which copies the mono input two times as the stereo channels. This method should have no stereo effect at all, thus outperforming it means the success of generating the sense of directions.
%
%
As the whole model of ours includes the separation training described in Sec.~\ref{sec:3.3.2}, we also evaluation the ablation of this module \textbf{(w/o sep.)}.
%
Table~\ref{table:exp1} shows the results of these methods on all metrics.

%Firstly we show the drawbacks of previous metrics. During training, 0.63s of audios are directly generated from the backbone according to one frame. However, the sliding window size for testing is set as 0.05s. The final outputs are averaged across the generated overlapped samples. We show an example of setting the sliding window to 0.63s during testing, named \textbf{Mono2Binaural (0.63s)}. The sliding window operation has no effect on Mono-Mono as the audios on a specific position are the same across clips. It can be seen from Table~\ref{table:exp1} that the numerical results of Mono2Binaural (0.63s) are even worse than Mono-Mono on STFT and ENV distances. 
%However, for most cases in the dataset, both camera-views and sound sources are stable. Thus the sensitiveness in these metrics is not affected by sound source positions. 
%Thus the sensitiveness of these metrics to sliding window size is not affected by sound source positions. 
%While on our metrics, the size of the sliding window has little influence on the final results. Mono-Mono, on the other hand, performs badly on our metrics as there is no location information. This proves the superiority of our metrics comparing with previous ones.

With no supervision, it is reasonable that our \emph{PseudoBinaural} cannot outperform the supervised setting. However, the fact that our model outperforms \emph{Mono-Mono} on all metrics proves the effectiveness of our proposed method. In line with previous work~\cite{zhou2020sep}, introducing the separation task in the training framework can further improve the overall performance of generated binaural audio.

\noindent\textbf{Augmentation to Binaural Audio Training.} 
%
Since our method just relies on the pseudo visual-stereo pairs, a natural idea is to leverage both pseudo data and recorded ones to boost the performance of the traditional fully-supervised approach. As demonstrated in the lower half of Table~\ref{table:exp1}, our method, denoted as \emph{Augment-PseudoBinaural}, can surpass the traditional setting \emph{Mono2Binaural}~\cite{gao20192} on all 5 metrics. 
%
Moreover, compared to \emph{Sep-Stereo}~\cite{zhou2020sep}, which incorporates extra data, we create pseudo pairs with the same set of collected data,
%separation task to do the augmentation, 
%our pseudo visual-stereo pairs share the similar stereo sensation as the recorded audio, 
providing more effective and complementary information to guide the training.
Consequently, our method outperforms theirs on both FAIR-Play and MUSIC-Stereo.
%
%The drawback of our method on the FAIR-Play dataset is caused by the nature of the room reverberations. Specifically, we observe on YT-MUSIC dataset, our results are very close to the supervised ones even with traditional metrics.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent\textbf{Cross-Dataset Evaluation.} 
%
We specifically show the results of cross-dataset evaluation in Table.~\ref{table:exp2} to prove that 1) supervised methods can easily overfit to a specific domain and 2) the generalization ability of our method. YT-MUSIC~\cite{morgado2018self} with special 360\degree videos and ambisonics sounds is also used for evaluation. Here we use the non-augmented version of \emph{PseudoBinaural} for evaluation.
For \emph{Mono2Binaural}, the model evaluated on FAIR-Play is trained on MUSIC-Stereo, and the model tested on MUSIC-Stereo and YT-MUSIC is trained on FAIR-Play.
During cross-testing on FAIR-Play and MUSIC-Stereo, the visual to angle mapping $f_{v2a}$ is defined in the frontal view. But when cross-testing on YT-MUSIC, the video is defined in the form of 360\degree. 

We can see from the table that our method stably outperforms \emph{Mono2Binaural} in all cross-dataset evaluations. The supervised method tends to perform badly when testing in a different domain, while our recording-free method generalizes well by training only on mono data.

% Table 3

%========================================================
\begin{table}[t] %\footnotesize
\setlength{\tabcolsep}{8pt}
\begin{center}
\caption{Ablation study on the number $K$ of mono videos to mix based on FAIR-Play dataset. Obviously, a fixed number $K$ cannot create diverse scenarios to guide the training sufficiently. Therefore, we set the $K$ as an empirical ratio $1:2:3 = 0.4:0.5:0.1$ for all the experiments.
}
\label{table:exp3}
\begin{tabular}{lccccc}
\toprule
$K$ & $\text{STFT} $ & $\text{ENV} $ & $\text{Mag} $ & $\mathcal{D}_{phase} $ & $\text{SNR} \uparrow $ \\
\midrule
1  &0.965 &0.143 &1.914 &1.483 &4.976 \\
2  &0.935 &0.141 &1.871 &1.480 &5.026 \\
3  &0.967 &0.142 &1.936 &1.527 &5.004 \\
1,2 &0.895 &0.136 &1.793 &1.479 &5.282 \\
1,2,3  &\textbf{0.878} &\textbf{0.134} &\textbf{1.768} &\textbf{1.467} & \textbf{5.316} \\

\bottomrule
\end{tabular}
\end{center}
\vspace{-12pt}
\end{table}
%========================================================

% \begin{figure*}[!t]
% 	\begin{center}
% 		\includegraphics[width=1\textwidth]{figs/user}
% 	\end{center}
% 	\vspace{-10pt}
% 	\caption{
% 		Qualitative results. (a) shows the results of our user studies. It can be seen that the users slightly prefer our unsupervised approach over supervised Mono2Binaural~\cite{gao20192}. (b) is the visualization of the activation maps of ours and Mono2Binaural. While the attention of theirs are more messy, the results of ours are more compact. We focus more on the sound sources. 
% 	}

% 	\label{fig:localization}
% 	\vspace{-5pt}
% \end{figure*}
\begin{figure*}[!t]
    \centering
        \subfloat[User Study]{
        \begin{minipage}[b]{.46\textwidth}
        \flushright
        \includegraphics[width=1\textwidth]{figs/user1.pdf}\\
        \includegraphics[width=1\textwidth]{figs/user2.pdf}\\
        \includegraphics[width=1\textwidth]{figs/user3.pdf}
        \end{minipage}
        }
        \subfloat[Activation Map]{
        \begin{minipage}[b]{.26\textwidth}
        \includegraphics[width=1\textwidth]{figs/b1.png}
        \centerline{\small{Mono2Binaural~\cite{gao20192}}}
        \end{minipage}
        \begin{minipage}[b]{.26\textwidth}
        \includegraphics[width=1\textwidth]{figs/b2.png}
        \centerline{Ours}
        \end{minipage}
        }
	\caption{
		Qualitative results. (a) shows the results of our user studies. It can be seen that the users slightly prefer our approach over supervised Mono2Binaural~\cite{gao20192}. (b) is the visualization of the activation maps of ours and Mono2Binaural. While the attention of theirs is messier, the results of ours are more compact. We focus more on sound sources. 
	}
    \label{fig:localization}
    \vspace{-10pt}
\end{figure*}

\noindent\textbf{Ablation Study.} 
%
The lower half of Table~\ref{table:exp1} presents our ablation studies on different binaural decoding schemes. 
As written in Sec.~\ref{sec:3.1.2}, binaural audios can be decoded directly from \emph{HRIR} or \emph{ambisonic}. It can be seen that our way of combining both leads to the best results.

When preparing pseudo visual-stereo pairs, the number of mono videos to mix is also another important hyperparameter for consideration. As shown in Table~\ref{table:exp3}, a fixed mixing number $K$ always fails to construct various training samples, introducing inconsistency with those naturally collected datasets. %, and leads to bad performance eventually. 
Hence, an empirical ratio of $1:2:3 = 0.4:0.5:0.1$ for the number $K$ is applied to ensure the diversity of generated visual-stereo pairs.

\subsection{Qualitative Results}
\noindent\textbf{User Study\footnote{Please refer to \url{https://sheldontsui.github.io/projects/PseudoBinaural} for demo videos.}.} 
%
In total 30 users with normal hearing participated in our study
% similar to ~\cite{gao20192} 
to perform the quality evaluation.  There are three sets of studies, each with 20 videos selected from the test set of FAIR-Play~\cite{gao20192} and MUSIC-Stereo~\cite{zhao2019sound}, most of which are duets. 1) The users are asked to watch one video and listen to the binaural audios generated by \emph{PseudoBinaural}, \emph{Mono2Binaural}~\cite{gao20192} or \emph{Mono-Mono}. The question is which one of the three methods creates the best stereo sensation. The results show the percentage of the users' \textbf{Stereo Preferences.} 2) The users are asked to listen to the audio generated by the above methods without viewing videos, and decide where is the specific instrument (left, right, or center). Ground truth audios are also included for reference. The results show the \textbf{Sound Localization Accuracy} of these methods. 3) A subjective \textbf{Ablation Study} is conducted to show the influence of different choices of binaural decoding methods. The users are asked to tell which decoding diagram, direct HRIR, ambisonic, or ours, creates the best 3D hearing experience. 

The results are shown in Fig~\ref{fig:localization} (a). From the first and second experiments, we can see that users find our method slightly better than supervised \emph{Mono2Binaural} on both the two measurements.
%There are also an amount of users prefer mono results, and 18\% of users cannot correctly perceive the source direction even on ground truth, which shows the uncertainties in human listeners.
This is enough to validate that our results are highly competitive to supervised methods in subjective evaluations, which is extremely important for auditory tasks. 
In the sound localization experiment, users can only achieve $81\%$ accuracy even given the ground-truth audio, which demonstrates the misguiding caused by the room reverberations.
The subjective ablation study shows that our decoding procedure apparently creates the best sense of hearing among all decoding choices.



\noindent\textbf{Visualization.} 
%
We also visualize the activation map generated by our method and \emph{Mono2Binaural}~\cite{gao20192} on the visual domain.
% The bright places are the salient regions in the feature map, which demonstrates that our network always focuses on the potential sound sources.
In Fig.~\ref{fig:localization} (b) we can see that \emph{PseudoBinaural} can successfully attend to sound sources while \emph{Mono2Binaural}~\cite{gao20192} would focus on less important areas. For example, their approach would attend to the ceiling for all three scenes shown, which is not the sound source. 

% \begin{table}[!t] %\footnotesize
% \begin{center}
% \caption{ablation study on decoding methods}
% \label{table:exp3}
% \begin{tabular}{lcccc}
% \toprule
%  & \multicolumn{4}{c}{FAIR-Play} \\
% \cmidrule(lr){2-5}
% decoding & $\text{STFT}$ & $\text{ENV}$ & $\text{Mag}_D$ & $\text{ENV}_D$ \\

% \midrule
% HRTF  &1.323 &0.172 &2.684 &0.156  \\
% ambisonic+direct  &1.358 &0.180 &2.753 &0.156  \\
% ambisonic+HRTF  &\textbf{1.293} &\textbf{0.163} &\textbf{2.565} &\textbf{0.156} \\

% \bottomrule
% \end{tabular}
% \end{center}
% \end{table}

